Mitigating Redundant Data Transfers for Mobile Web Applications via App-Specific Cache Space

Redundant transfer of resources is a critical issue for compromising the performance of mobile Web applications (a.k.a., apps) in terms of data traffic, load time, and even energy consumption. Evidence shows that the current cache mechanisms are far from satisfactory. With lessons learned from how native apps manage their resources, in this paper, we propose the ReWAP approach to fundamentally reducing redundant transfers by restructuring the resource loading of mobile Web apps. ReWAP is based on an efficient mechanism of resource packaging where stable resources are encapsulated and maintained into a package, and such a package shall be loaded always from the local storage and updated by explicitly refreshing. By retrieving and analyzing the update of resources, ReWAP maintains resource packages that can accurately identify which resources can be loaded from the local storage for a considerably long period. ReWAP also provides a wrapper for mobile Web apps to enable loading and updating resource packages in the local storage as well as loading resources from resource packages. ReWAP can be easily and seamlessly deployed into existing mobile Web architectures with minimal modifications, and is transparent to end-users. We evaluate ReWAP based on continuous 15-day access traces of 50 mobile Web apps that suffer heavily from the problem of redundant transfers. Compared to the original mobile Web apps with cache enabled, ReWAP can significantly reduce the data traffic, with the median saving up to 51%. In addition, ReWAP can incur only very minor runtime overhead of the client-side browsers.

==> biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/Xuanzhe}}]{Xuanzhe~Liu}
is an associate professor in the School of Electronics Engineering
and Computer Science, Peking University, Beijing, China. His research interests
are in the area of services computing, mobile computing, web-based systems, and big data analytic.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/mayun}}]{Yun~Ma}
is a Ph.D student in the School of Electronics Engineering
and Computer Science of Peking University, Beijing, China.  His research interests include services computing and web engineering.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/XinyangWang}}]{Xinyang Wang}
received his Bachelor degree in computer science from Peking University in 2015. Now he is pursing the master degree of computer science in University of Washington. His field of interest includes mobile network, wearable computing, and software engineering.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1.2in,height=1.25in,clip,keepaspectratio]{figure/yunxin}}]{Yunxin~Liu} is a lead researcher in Microsoft Research Asia. He received my Ph.D. in computer science from Shanghai Jiao Tong University in 2011 (through the SJTU-MSRA joint PhD program). His current research interests include mobile systems and networking.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1.2in,height=1.25in,keepaspectratio]{figure/taoxie}}]{Tao~Xie} is an Associate Professor in the Department of Computer Science at the University of Illinois at Urbana-Champaign, USA. His research interests are software testing, program analysis, software analytics, software security, and educational software engineering. He is a senior member of IEEE.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/Huanggang}}]{Gang~Huang} is now
a full professor in Institute of Software, Peking University.
His research interests are in the area of middleware of cloud computing and mobile computing. He is a member of IEEE.
\end{IEEEbiography}
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/meihong}}]{Hong~Mei}
%is a full professor of School of Electronics Engineering and
%Computer Science, Peking University, Beijing, China. His current research interests are in the area of software engineering and operating systems.
%Hong Mei is a member of the Expert Committee for Information Technology of State 863 High-Tech Program, a chief scientist of State 973 Fundamental Research Program. He is the Member of Chinese Academy of Sciences, and the Fellow of China Computer Federation (CCF). He is a fellow of the IEEE.
%\end{IEEEbiography}

